Cutting Plane Selection with Analytic Centers and Multiregression

Cutting planes are a crucial component of state-of-the-art mixed-integer programming solvers, with the choice of which subset of cuts to add being vital for solver performance. We propose new distance-based measures to qualify the value of a cut by quantifying the extent to which it separates relevant parts of the relaxed feasible set. For this purpose, we use the analytic centers of the relaxation polytope or of its optimal face, as well as alternative optimal solutions of the linear programming relaxation. We assess the impact of the choice of distance measure on root node performance and throughout the whole branch-and-bound tree, comparing our measures against those prevalent in the literature. Finally, by a multi-output regression, we predict the relative performance of each measure, using static features readily available before the separation process. Our results indicate that analytic center-based methods help to significantly reduce the number of branch-and-bound nodes needed to explore the search space and that our multiregression approach can further improve on any individual method.

==> response_to_reviewers.tex <==
% Reviewer 1 -

% For nodes we do this already. For time we do have promising results for particular instance classes that we hope to present at the conference. For general MIP it's ongoing research.

% Reviewer 2 -

% Put results for all methods minus the time spent in cut selection. Get percent of time spent in cut selection for the instances. We wanted to avoid overselling as the time spent is an integral part of the solving process. (Put the avoid overselling in the response)

% Example sentence: On average the analytic center calls take x\% of the root node solve time, with extreme cases reaching up to y\%. This is contrast to the standard method efficacy, which only reaches up to x\%.

% Mention explicitly the amount of dual degeneracy in MIPLIB from Geralds paper.

% Put in some sentence in the paper (steal number from Gerald + Timo). Write in the response the number explicitly.

% Reviewer 3 -

% Do they mean selection instead of generation? If they mean selection, then we believe in general the answer is no, the extra time is not worth it, but that there are a huge amount fo cases where it is. Our experiments do not go past the root ndoe for cuts, but all commercial MIP solvers and SCIP do add cuts after the root node. For generation, link the zero half computational study, which suggests that spamming diverse sets of cheaper cuts is better on average than expensive cuts (for generation).

% Sentences: For the amount of overhead see our response to reviewer 2. For the question of whether our approach is worth including in a default solver, see the response to reviewer 1. It's very nice to see that the reviewers raised similar questions. 

% Link to Tobi's thesis. Complementarity means orthogonality? Overall to the best of our knowledge this not the most effective method. Comparing all cuts to each other would be quadratic and this is one of the reasons it's not done. (Mention good / bad score in SCIP that uses orthogonality)

We thank the reviewers for their thorough reviews and helpful comments on our work. We are excited to see that the reviewers find our work interesting and valuable.

Response to rebuttal of Reviewer 1:

- We believe the output of our trained SVR is itself a static rule defined by multiple polynomials of the instance features, which does improve performance over a simplified version of default w.r.t. the number of nodes (It is however not a constant rule which uses the same ratio of measures for each instance). The static rule motivation is exactly what prompted us to choose a simple to implement and interpretable machine learning model. To truly create a new static selection rule that would be enabled by default in SCIP, one would need a larger computational study with combinations of measures, many of which are not distance-based. This is indeed part of our ongoing research. In the meantime, we have some promising results for particular instance classes that we hope to present at CPAIOR.

Response to rebuttal of Reviewer 2:

- We agree with the point raised on the time spent in the analytic center. We'd like to clarify that we avoided making conclusions from data with the time removed, as it might appear in us overselling our proposed measures due to time spent being an integral part of the solving process in practice. We have added a sentence in the computational section (4.1) to give orders of magnitude on the time spent:

"It should be noted, however, that on average a-eff takes 32 percent of the root node processing time and a-dcd takes 25, which is in contrast to eff, which only takes 0.8 percent."

- There have been studies done on dual degeneracy and the frequency in which it appears. A study that we cite, "An exploratory computational analysis of dual degeneracy in mixed-integer programming", which we will make clearer in the paper, uses a mixture of older MIPLIB data sets and COR@L, and provides statistics on the ratio at which dual degeneracy appears after processing the root node (presolve and cutting rounds). The following sentence on the frequency of dual degeneracy in practice has been added to the paper:

"We note that 90.4 percent of cuts have infeasible projections when scoring by eff, and that previous studies, see (An exploratory computational analysis of dual degeneracy in mixed-integer programming
), identify an 87.5 percent occurrence rate of some level of dual degeneracy of the final root node LP in standard benchmark instances, confirming the practical geometric limitations of efficacy presented in Section 3.3."

- Thanks for pointing out the minor issues as well, especially the error in Figure 3! We have fixed the issues raised, following the suggestions when given. For the question on a-dcd vs dcd:

Cutting toward the central point is an effective tool against dual degeneracy, which is the Achilles' heel of some instances. Our original intuition, however, was that a-eff would be a more effective measure. We also were surprised at the difference between approx-a-dcd and a-dcd, which hints at the analytic center moving significantly, with some level of centrality being lost.
For dcd, we observed that it was surprisingly poor at the root node, despite obviously paying off in the longer solving process. We believe it too strongly biases one direction, which is often somewhat extreme (and it doesn't update during the cutting rounds like a-dcd does). This direction is then simply a poor choice for some instances and keeps undervaluing some necessary cuts. We have wondered though if this would be true for all optimal solutions (in the case multiple exist). 


Response to rebuttal of Reviewer 3:

- We are unsure if the reviewer meant selection instead of generation for their first point. 
If they meant selection: We cannot make the blanket statement "additional time spent in selection is preferable for the solving process". While such a statement is more likely to be true for the number of nodes, it does not translate to the solve time as our paper showed. For this work we restricted ourselves to the root node for cut selection, however, all commercial solvers and SCIP do perform cut generation and selection past the root node by default.
If they meant generation: Older computational studies -- we specifically point to "Embedding \{0,1/2\}-Cuts in a Branch-and-Cut Framework: A Computational Study" -- conclude that it is more effective to produce a large amount of cheaper cuts than a small amount of expensive cuts. These conclusions are not restricted to the root node. All such results to our knowledge come from computational results and always rely on an appropriate filtering algorithm to ensure mass amounts of similar cheap cuts are not added. 

- We assume the reviewer refers to orthogonality when using complementarity. From our experiments, we know that the sets of generated cuts have a significant amount of mutual orthogonality. We refer to the thesis "Constraint integer programming" for more results on this. We will also add that to the best of our knowledge scoring cuts by their orthogonality is tricky, and pairwise comparing all cuts results in a quadratic algorithm. If the reviewer meant an approach of many different measures, then we agree that incorporating multiple measures would be helpful. Our study looked at distance measures in isolation, however, if we were to deploy to a MIP solver, we would recommend integrating non-distance-based measures to complement the scoring (or ranking) process, and potentially the filtering process.

We hope our comments help to clarify the questions about our work and support the evaluation process.
